On wall-crossing coordinates in Cerf theory

We relate Bruhat numbers in real Morse theory to cluster variables in braid varieties. This provides instances of wall-crossing coordinates in the study of Cerf diagrams.

==> 3_Questions.tex <==
\section{Remarks}\label{sec:questions}

Here follow a few comments around \maintheoref.
%Despite their verbose and contentless nature, we hope some of them can motivate further work on the subject.

\subsection{Cluster structures in the general case} The braid variety $X(w_0\beta)$ is closely related to the augmentation stack of the Legendrian contact dg-algebra of the Legendrian link $\La_\beta\sse(\R^3,\xi_\st)$ whose front is $\pi_\beta$, understood as a cooriented front projection, cf.~\cite[Theorem 1.1.(iv)]{CGGS} or \cite[Section 6.2.1]{Casals_CBMSNotes}. For more general Legendrian links $\La_\beta\sse(\R^3,\xi_\st)$, it is yet to be proven that the coordinate ring of the augmentation stack is a cluster algebra: I do conjecture this to be true. It follows from \cite{CGGLSS} that this is the case for any $(-1)$-closure of a positive braid of the form $w_0\beta$, and it can be proven by entirely contact methods by using \cite{CasalsWeng}.

For an arbitrary Legendrian link $\La_\beta\sse(\R^3,\xi_\st)$ given by a generating family, \maintheoref provides a first hint at a proof for the general fact that all augmentations varieties should be cluster, both these words being appropriately understood. Indeed, they key idea would be to use Bruhat numbers in order to construct the cluster variables, then potentially following these steps:

\begin{enumerate}
    \item For each switch of the associated normal ruling, declare the (putative) cluster variable to be the appropriate product of Bruhat numbers for the Morse function at the right of that crossing, the product of Bruhat numbers being chosen according to the recipe in \cite{CGGLSS}. In particular, if the degree-0 differential is in the top Bruhat cell, this coincides with the product in \maintheoref and, in general, it is some monomial on generalized minors and the cluster variables constructed so far to the left.\\

    \item Use \cite{casals2024positivemicrolocalholonomiesglobally} with an $\L$-compressing system associated to the ruling to argue that these products are globally regular on the augmentation variety.\\

    \item Determine the quiver via the same method as for the Deodhar cluster structures, \cite[Section 5.2]{casals2025comparingclusteralgebrasbraid}. Specifically, show that the symplectic 2-form coming from Sabloff duality is in normal Darboux form with respect to these products of Bruhat numbers.
\end{enumerate}

\noindent It would also be desirable to obtain the quiver via an $\L$-compressing system, as this would be more explicit. It would be valuable to have progress in any of these steps above for a general Legendrian link, even if just building an $\L$-compressing system, or naming an initial seed.

\subsection{A moduli of 1-parametric families of Morse functions} There is a precise connection between parametric Morse theory and the study of Legendrian submanifolds, from normal rulings, as introduced and studied by D.~Fuchs, P.~Pushkar and Y.~Chekanov and their collaborators, to generating families for Legendrian submanifolds and their associated invariants, as developed by many, including C.~Viterbo, D.~Th\'eret, and L.~Traynor, see e.g.~\cite{BourgeoisSabloffTraynor15_GeneratingFunctions,EliashbergGromov_GeneratingFamilies} and references therein.\\

From the viewpoint of Cerf theory, it could be enlightening to be able to rigorously name a reasonably behaved space of all the 1-parametric families of Morse functions with a given Cerf diagram, and understand how that space varies as the Cerf diagram varies, e.g.~ under front homotopies or surgeries.
